Privacy-Enhancing Technologies for Artificial Intelligence-Enabled Systems

Artificial intelligence (AI) models introduce privacy vulnerabilities to systems. These vulnerabilities may impact model owners or system users; they exist during model development, deployment, and inference phases, and threats can be internal or external to the system. In this paper, we investigate potential threats and propose the use of several privacy-enhancing technologies (PETs) to defend AI-enabled systems. We then provide a framework for PETs evaluation for a AI-enabled systems and discuss the impact PETs may have on system-level variables.

==> references.tex <==
@Techreport{IBM2022,
  author =       "",
  year =         "2022",
  title =        "IBM Global AI Adoption Index 2022",
  institution =  "IBM Corporation",
  type =         "IBM Technology Adoption Report",
  number =       "",
  address =      "Armonk, NY",
  month =        "",
  note =         "",
}


@article{Exposed2017,
author = {Dwork, Cynthia and Smith, Adam and Steinke, Thomas and Ullman, Jonathan},
title = {Exposed! A Survey of Attacks on Private Data},
journal = {Annual Review of Statistics and Its Application},
volume = {4},
number = {1},
pages = {61-84},
year = {2017},
doi = {10.1146/annurev-statistics-060116-054123},

URL = { 
    
        https://doi.org/10.1146/annurev-statistics-060116-054123
    
    

},
eprint = { 
    
        https://doi.org/10.1146/annurev-statistics-060116-054123
    
    

}
,
    abstract = { Privacy-preserving statistical data analysis addresses the general question of protecting privacy when publicly releasing information about a sensitive dataset. A privacy attack takes seemingly innocuous released information and uses it to discern the private details of individuals, thus demonstrating that such information compromises privacy. For example, re-identification attacks have shown that it is easy to link supposedly de-identified records to the identity of the individual concerned. This survey focuses on attacking aggregate data, such as statistics about how many individuals have a certain disease, genetic trait, or combination thereof. We consider two types of attacks: reconstruction attacks, which approximately determine a sensitive feature of all the individuals covered by the dataset, and tracing attacks, which determine whether or not a target individual's data are included in the dataset. We also discuss techniques from the differential privacy literature for releasing approximate aggregate statistics while provably thwarting any privacy attack. }
}





@article{Pitro19,
title = {A taxonomy and survey of attacks against machine learning},
journal = {Computer Science Review},
volume = {34},
pages = {100199},
year = {2019},
issn = {1574-0137},
doi = {https://doi.org/10.1016/j.cosrev.2019.100199},
url = {https://www.sciencedirect.com/science/article/pii/S1574013718303289},
author = {Nikolaos Pitropakis and Emmanouil Panaousis and Thanassis Giannetsos and Eleftherios Anastasiadis and George Loukas},
keywords = {Machine learning, Attacks, Taxonomy, Survey},
abstract = {The majority of machine learning methodologies operate with the assumption that their environment is benign. However, this assumption does not always hold, as it is often advantageous to adversaries to maliciously modify the training (poisoning attacks) or test data (evasion attacks). Such attacks can be catastrophic given the growth and the penetration of machine learning applications in society. Therefore, there is a need to secure machine learning enabling the safe adoption of it in adversarial cases, such as spam filtering, malware detection, and biometric recognition. This paper presents a taxonomy and survey of attacks against systems that use machine learning. It organizes the body of knowledge in adversarial machine learning so as to identify the aspects where researchers from different fields can contribute to. The taxonomy identifies attacks which share key characteristics and as such can potentially be addressed by the same defence approaches. Thus, the proposed taxonomy makes it easier to understand the existing attack landscape towards developing defence mechanisms, which are not investigated in this survey. The taxonomy is also leveraged to identify open problems that can lead to new research areas within the field of adversarial machine learning.}
}

@misc{mitre,
    title = {ATLAS Matrix},
    author= {MITRE},
    year="[n.d.]",
    url = "https://atlas.mitre.org/matrices/ATLAS/"}

@misc{zhang2023does,
      title={How Does a Deep Learning Model Architecture Impact Its Privacy? A Comprehensive Study of Privacy Attacks on CNNs and Transformers}, 
      author={Guangsheng Zhang and Bo Liu and Huan Tian and Tianqing Zhu and Ming Ding and Wanlei Zhou},
      year={2023},
      eprint={2210.11049},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}


@misc{uci-privacy-confidentiality,
  author        = "UCI Office of Research",
  year          = "[n.d.]",
  title         = "Privacy and Confidentiality",
  url           = "https://research.uci.edu/human-research-protections/research-subjects/privacy-and-confidentiality/",
}

@misc{nist-confidentiality,
  author        = "National Cybersecurity Center of Excellence, NIST",
  year          = "[n.d.]",
  title         = "Data Confidentiality: Identifying and Protecting Assets",
  url           = "https://www.nccoe.nist.gov/data-confidentiality-identifying-and-protecting-assets-and-data-against-data-breaches",
}

@misc{edtech-confidentiality,
  author        = "Mike Chapple",
  year          = "2019",
  title         = "Privacy vs Confidentiality vs Security: What's the Difference?",
  journal       = "EdTech",
  url           = "https://edtechmagazine.com/higher/article/2019/10/security-privacy-and-confidentiality-whats-difference",
}

@misc{dol-pii,
  author        = "U.S. Department of Labor",
  year          = "[n.d.]",
  title         = "Guidance on the Protection of Personal Identifiable Information",
  url           = "https://www.dol.gov/general/ppii", 
}

@misc{hipaa,
  author        = "U.S. Department of Health and Human Services",
  year          = "[n.d.]",
  title         = "Summary of the HIPAA Privacy Rule",
  url           = "https://www.hhs.gov/hipaa/for-professionals/privacy/laws-regulations/index.html", 
}

@misc{gdpr,
  author        = "Ben Wolford",
  year          = "[n.d.]",
  title         = "What is GDPR, the EU’s new data protection law?",
  url           = "https://gdpr.eu/what-is-gdpr/", 
}

@misc{adversarial-attacks,
      title={Adversarial Attacks on Neural Network Policies}, 
      author={Sandy Huang and Nicolas Papernot and Ian Goodfellow and Yan Duan and Pieter Abbeel},
      year={2017},
      eprint={1702.02284},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{threats-breakdown,
  author        = "Nick Bradley",
  year          = "2015",
  title         = "The Threat Is Coming From Inside the Network: Insider Threats Outrank External Attacks",
  url           = "https://securityintelligence.com/the-threat-is-coming-from-inside-the-network/", 
}

@misc{DARPA,
    author = "DARPA",
    year = "2020",
    title = "Data Protection in Virtual Environments (DPRIVE)", 
    publisher = "Microsystems Technology Office",
    number = "HR001120S0032"
}

@misc{chatgpt,
  author        = "OpenAI",
  year          = "2022",
  title         = "Introducing ChatGPT",
  url           = "https://openai.com/blog/chatgpt", 
}

@inproceedings{HERACLES,
author = {Cammarota, Rosario},
title = {Intel HERACLES: Homomorphic Encryption Revolutionary Accelerator with Correctness for Learning-Oriented End-to-End Solutions},
year = {2022},
isbn = {9781450398756},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3560810.3565290},
doi = {10.1145/3560810.3565290},
abstract = {In spite strong advances in confidential computing technologies to protect data, the status is that data is encrypted while temporarily not in use and unencrypted during computation. The inability to keep data encrypted during computation can inhibit the ability to fully share and extract the maximum value out of data, e.g., via statistical and machine learning methods with the additional risk of third-party data leakage. Fully Homomorphic Encryption (FHE) enables users to delegate computation to the cloud by enabling the cloud to process users' encrypted inputs without decryption and return encrypted output to the intended recipients. The adoption of FHE by the industry has been slow. First, processing encrypted data incurs a huge performance tax even for simple operations - ciphertexts operations can be several orders of magnitude slower with respect to cleartext operations on existing hardware. Second, there is lack of automation tools for translating data and applications to enable FHE. Third, there is lack of standards and best practices for FHE secure deployment in combination with other confidential computing techniques. The DARPA DPRIVE program [1] is the first publicly visible program aiming to build a platform to accelerate FHE and a path to their commercialization, for their use in healthcare, communication (5G to XG), and cloud computing. The program represents a steppingstone toward FHE adoption. Under the DARPA DPRIVE program, Intel® is designing a new type of computer architecture to reduce the performance tax currently associated with FHE. Intel® collaborates with Microsoft® Azure Global in realization of the project [2]. The design includes flexible arithmetic circuits for algebraic lattices with unprecedented vector parallelism and data transfer capacity between vector slots, to increase ciphertext processing speed, coupled with near-memory computation, to reduce data movement. The software stack leverages the Microsoft® SEAL library [3] augmented the BGV mechanism including bootstrapping [4], and automatic translation tools to explore trade-offs in algorithmic optimization and data encoding to fit the performance requirements [5]. When fully realized, the HERACLES platform will deliver a massive improvement in executing FHE workloads over existing CPU-driven systems, potentially reducing ciphertext processing time by five orders of magnitude. Beyond the new hardware and software stack, Intel® work with international standard bodies to develop standards for and best practices for FHE secure deployment [6] and invests in academic research to advance both theory and application [7].},
booktitle = {Proceedings of the 2022 on Cloud Computing Security Workshop},
pages = {3},
numpages = {1},
keywords = {fully homomorphic encryption, bootstrapping, privacy-enhancing cryptography, asic},
location = {Los Angeles, CA, USA},
series = {CCSW'22}
}



@inproceedings{BTS,
author = {Kim, Sangpyo and Kim, Jongmin and Kim, Michael Jaemin and Jung, Wonkyung and Kim, John and Rhu, Minsoo and Ahn, Jung Ho},
title = {BTS: An Accelerator for Bootstrappable Fully Homomorphic Encryption},
year = {2022},
isbn = {9781450386104},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3470496.3527415},
doi = {10.1145/3470496.3527415},
abstract = {Homomorphic encryption (HE) enables the secure offloading of computations to the cloud by providing computation on encrypted data (ciphertexts). HE is based on noisy encryption schemes in which noise accumulates as more computations are applied to the data. The limited number of operations applicable to the data prevents practical applications from exploiting HE. Bootstrapping enables an unlimited number of operations or fully HE (FHE) by refreshing the ciphertext. Unfortunately, bootstrapping requires a significant amount of additional computation and memory bandwidth as well. Prior works have proposed hardware accelerators for computation primitives of FHE. However, to the best of our knowledge, this is the first to propose a hardware FHE accelerator that supports bootstrapping as a first-class citizen.In particular, we propose BTS --- Bootstrappable, Technology-driven, Secure accelerator architecture for FHE. We identify the challenges of supporting bootstrapping in the accelerator and analyze the off-chip memory bandwidth and computation required. In particular, given the limitations of modern memory technology, we identify the HE parameter sets that are efficient for FHE acceleration. Based on the insights gained from our analysis, we propose BTS, which effectively exploits the parallelism innate in HE operations by arranging a massive number of processing elements in a grid. We present the design and microarchitecture of BTS, including a network-on-chip design that exploits a deterministic communication pattern. BTS shows 5,556\texttimes{} and 1,306\texttimes{} improved execution time on ResNet-20 and logistic regression over a CPU, with a chip area of 373.6mm2 and up to 163.2W of power.},
booktitle = {Proceedings of the 49th Annual International Symposium on Computer Architecture},
pages = {711–725},
numpages = {15},
keywords = {technology-driven, accelerator, fully homomorphic encryption, bootstrapping, CKKS},
location = {New York, New York},
series = {ISCA '22}
}



@article{samsung,
  author        = "Mark Gurman",
  year          = "2023",
  title         = "Samsung Bans Staff’s AI Use After Spotting ChatGPT Data Leak",
  journal       = "Bloomberg",
  url           = "https://www.bloomberg.com/news/articles/2023-05-02/samsung-bans-chatgpt-and-other-generative-ai-use-by-staff-after-leak", 
}

@article{northrop-grumman,
    author = "Lindsay Ellis",
    title = "ChatGPT Can Save You Hours at Work. Why Are Some Companies Banning It?",
    journal = "Wall Street Journal",
    year = "2023"
}

@misc{aws-nitro-enclave,
  author        = "Amazon Web Services",
  year          = "[n.d.]",
  title         = "AWS Nitro Enclaves",
  url           = "https://aws.amazon.com/ec2/nitro/nitro-enclaves/", 
}

@misc{azure-sgx-enclave,
  author        = "Microsoft Azure",
  year          = "2022",
  title         = "SGX enclaves",
  url           = "https://learn.microsoft.com/en-us/azure/confidential-computing/confidential-computing-enclaves", 
}

@article{chatgpt-size,
    author = "Alex Hughes",
    title = "ChatGPT: Everything you need to know about OpenAI's GPT-4 tool",
    journal = "BBC Science Focus",
    year = "2023",
    url = "https://www.sciencefocus.com/future-technology/gpt-3"
}

@misc{bert-size,
      title={BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding}, 
      author={Jacob Devlin and Ming-Wei Chang and Kenton Lee and Kristina Toutanova},
      year={2019},
      eprint={1810.04805},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@INPROCEEDINGS{netflix,
  author={Narayanan, Arvind and Shmatikov, Vitaly},
  booktitle={2008 IEEE Symposium on Security and Privacy (sp 2008)}, 
  title={Robust De-anonymization of Large Sparse Datasets}, 
  year={2008},
  volume={},
  number={},
  pages={111-125},
  doi={10.1109/SP.2008.33}
}

@article{tesla-attack,
    author = "Karen Hao",
    title = "Hackers trick a Tesla into veering into the wrong lane",
    journal = "MIT Technology Review",
    year = "2019",
    url = "https://www.technologyreview.com/2019/04/01/65915/hackers-trick-teslas-autopilot-into-veering-towards-oncoming-traffic/"
}

@article{fl-gla-1,
    author = "Haimei Gong and Liangjun Jiang and Xiaoyang Liu and Yuanqi Wang and Omary Gastro and Lei Wang and Ke Zhang and Zhen Guo",
    title = "Gradient leakage attacks in federated learning",
    journal = "Artificial Intelligence Review",
    year = "2023",
    doi = "https://doi.org/10.1007/s10462-023-10550-z"
}

@ARTICLE{fl-gla-2,
  author={Haomiao Yang and Mengyu Ge and Dongyun Xue and Kunlan Xiang and Hongwei Li and Rongxing Lu},
  journal={IEEE Network}, 
  title={Gradient Leakage Attacks in Federated Learning: Research Frontiers, Taxonomy and Future Directions}, 
  year={2023},
  volume={},
  number={},
  pages={1-8},
  doi={10.1109/MNET.001.2300140}
}

@incollection{tee-attestation,
	doi = {10.1007/978-3-031-16092-9_7},
	url = {https://doi.org/10.1007%2F978-3-031-16092-9_7},
	year = 2022,
	publisher = {Springer International Publishing},
	pages = {95--113},
	author = {Jämes M{\'{e}
}n{\'{e}}trey and Christian Göttel and Anum Khurshid and Marcelo Pasin and Pascal Felber and Valerio Schiavoni and Shahid Raza},
	title = {Attestation Mechanisms for~Trusted Execution Environments Demystified},
	booktitle = {Distributed Applications and Interoperable Systems}
}

@article{fhe-inference,
    author = "Liv d'Aliberti and Joe Kovba and Manbir Gulati and Sami Hoda and Ben Snively",
    title = "Enable fully homomorphic encryption with Amazon SageMaker endpoints for secure, real-time inferencing",
    journal = "AWS Machine Learning Blog",
    year = "2023",
    url = "https://aws.amazon.com/blogs/machine-learning/enable-fully-homomorphic-encryption-with-amazon-sagemaker-endpoints-for-secure-real-time-inferencing/"
}

@article{synthetic-data-generation,
    author = "Gerard Andrews",
    title = "What is Synthetic Data?",
    journal = "NVIDIA",
    year = "2021",
    url = "https://blogs.nvidia.com/blog/2021/06/08/what-is-synthetic-data/"
}

@article{differential-privacy,
    author = "Joseph Near and David Darais and Kaitlin Boeckl",
    title = "Differential Privacy for Privacy-Preserving Data Analysis",
    journal = "Cybersecurity Insights (A NIST Blog)",
    year = "2020",
    url = "https://www.nist.gov/blogs/cybersecurity-insights/differential-privacy-privacy-preserving-data-analysis-introduction-our"
}

@INPROCEEDINGS{split-learning,
  author={Jihyeon Ryu and Dongho Won and Youngsook Lee},
  booktitle={2022 16th International Conference on Ubiquitous Information Management and Communication (IMCOM)}, 
  title={A Study of Split Learning Model}, 
  year={2022},
  volume={},
  number={},
  pages={1-4},
  doi={10.1109/IMCOM53663.2022.9721798}
}

@article{us-census,
    author = "The Population Reference Bureau and
the U.S. Census Bureau’s 2020 Census Data Products and Dissemination Team",
    title = "Why the Census Bureau Chose Differential Privacy",
    journal = "U.S. Census Bureau",
    year = "2023",
    url = "https://www2.census.gov/library/publications/decennial/2020/census-briefs/c2020br-03.pdf"
}

@article{iso-fhe-standard,
    author = "ISO",
    title = "ISO/IEC WD 18033-8",
    year = "2023",
    url = "https://www.iso.org/standard/83139.html"
}

@techreport{fhe-standard,
 author = {Martin Albrecht and Melissa Chase and Hao Chen and Jintai Ding and Shafi Goldwasser and Sergey Gorbunov and Shai Halevi and Jeffrey Hoffstein and Kim Laine and Kristin Lauter and Satya Lokam and Daniele Micciancio and Dustin Moody and Travis Morrison and Amit Sahai and Vinod Vaikuntanathan},
 title = {Homomorphic Encryption Security Standard},
 institution= {HomomorphicEncryption.org},
 publisher = {HomomorphicEncryption.org},
 address = {Toronto, Canada},
 year = {2018},
 month = {November}
 }

@misc{intel-sgx,
    author = "Intel",
    title = "Intel® Software Guard Extensions (Intel® SGX)",
    journal = "",
    year = "[n.d.]",
    url = "https://www.intel.com/content/www/us/en/architecture-and-technology/software-guard-extensions.html"
}

@ARTICLE{CKKS-Network,
  author={Lee, Eunsang and Lee, Joon-Woo and Kim, Young-Sik and No, Jong-Seon},
  journal={IEEE Access}, 
  title={Optimization of Homomorphic Comparison Algorithm on RNS-CKKS Scheme}, 
  year={2022},
  volume={10},
  number={},
  pages={26163-26176},
  doi={10.1109/ACCESS.2022.3155882}}

@article{intel-fhe,
    author = "Ro Cammarota",
    title = "Intel Labs Continues Focused Research and Standards Efforts to Make FHE Viable",
    journal = "Intel",
    year = "2023"
}

@misc{intel-remote-attestation,
    author = "Intel",
    title = "Strengthen Enclave Trust with Attestation",
    journal = "",
    year = "[n.d.]",
    url = "https://www.intel.com/content/www/us/en/developer/tools/software-guard-extensions/attestation-services.html"
}

@article{duality,
    author = "Kurt Rohloff",
    title = "Homomorphic Encryption – Making it Real",
    journal = "Duality",
    year = "2017",
    url = "https://dualitytech.com/blog/homomorphic-encryption-making-it-real/"
}

@article{duality-openfhe,
    author = "Kurt Rohloff",
    title = "Duality Advances Homomorphic Encryption Landscape with OpenFHE",
    journal = "Duality",
    year = "2022",
    url = "https://dualitytech.com/blog/duality-advances-homomorphic-encryption-landscape-with-openfhe/"
}

@misc{enisa,
    author = "ENISA",
    title = "ENISA’s PETs Maturity Assessment Repository",
    journal = "",
    year = "2019",
    url = "https://www.enisa.europa.eu/publications/enisa2019s-pets-maturity-assessment-repository"
}

@article{wsj-tiktok-attack,
    author = "WSJ Staff",
    title = "Inside TikTok’s Algorithm: A WSJ Video Investigation",
    journal = "Wall Street Journal",
    year = "2021",
    url = "https://www.wsj.com/articles/tiktok-algorithm-video-investigation-11626877477"
}

@misc{chatgpt-petaflops,
      title={Language Models are Few-Shot Learners}, 
      author={Tom B. Brown and Benjamin Mann and Nick Ryder and Melanie Subbiah and Jared Kaplan and Prafulla Dhariwal and Arvind Neelakantan and Pranav Shyam and Girish Sastry and Amanda Askell and Sandhini Agarwal and Ariel Herbert-Voss and Gretchen Krueger and Tom Henighan and Rewon Child and Aditya Ramesh and Daniel M. Ziegler and Jeffrey Wu and Clemens Winter and Christopher Hesse and Mark Chen and Eric Sigler and Mateusz Litwin and Scott Gray and Benjamin Chess and Jack Clark and Christopher Berner and Sam McCandlish and Alec Radford and Ilya Sutskever and Dario Amodei},
      year={2020},
      eprint={2005.14165},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{openfhe,
      author = {Ahmad Al Badawi and Jack Bates and Flavio Bergamaschi and David Bruce Cousins and Saroja Erabelli and Nicholas Genise and Shai Halevi and Hamish Hunt and Andrey Kim and Yongwoo Lee and Zeyu Liu and Daniele Micciancio and Ian Quah and Yuriy Polyakov and Saraswathy R.V. and Kurt Rohloff and Jonathan Saylor and Dmitriy Suponitsky and Matthew Triplett and Vinod Vaikuntanathan and Vincent Zucca},
      title = {OpenFHE: Open-Source Fully Homomorphic Encryption Library},
      howpublished = {Cryptology ePrint Archive, Paper 2022/915},
      year = {2022},
      note = {\url{https://eprint.iacr.org/2022/915}},
      url = {https://eprint.iacr.org/2022/915}
}

@misc{record-linkage,
      title={Privacy-preserving Deep Learning based Record Linkage}, 
      author={Thilina Ranbaduge and Dinusha Vatsalan and Ming Ding},
      year={2022},
      eprint={2211.02161},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}

@misc{data-poisoning,
      title={Machine Learning Security against Data Poisoning: Are We There Yet?}, 
      author={Antonio Emanuele Cinà and Kathrin Grosse and Ambra Demontis and Battista Biggio and Fabio Roli and Marcello Pelillo},
      year={2023},
      eprint={2204.05986},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}

@misc{tee-inference,
      title={Privacy-Preserving Inference in Machine Learning Services Using Trusted Execution Environments}, 
      author={Krishna Giri Narra and Zhifeng Lin and Yongqin Wang and Keshav Balasubramaniam and Murali Annavaram},
      year={2019},
      eprint={1912.03485},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{iso-ai,
    author = "ISO",
    title = "ISO/IEC TR 27563:2023",
    year = "2023",
    url = "https://www.iso.org/standard/80396.html"
}

@misc{dlp,
    author = "Microsoft",
    title = "What is data loss prevention (DLP)?",
    journal = "",
    year = "[n.d.]",
    url = "https://www.microsoft.com/en-us/security/business/security-101/what-is-data-loss-prevention-dlp"
}

@article{ueba,
    author = "Nick Cavalancia",
    title = "User and Entity Behavior Analytics (UEBA) explained",
    journal = "AT\&T",
    year = "2020",
    url = "https://cybersecurity.att.com/blogs/security-essentials/user-entity-and-behavior-analytics-explained"
}

@misc{fhe-speed,
      title={Comprehensive Performance Analysis of Homomorphic Cryptosystems for Practical Data Processing}, 
      author={Vasily Sidorov and Ethan Yi Fan Wei and Wee Keong Ng},
      year={2022},
      eprint={2202.02960},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}

@misc{gpt2extraction,
      title={Extracting Training Data from Large Language Models}, 
      author={Nicholas Carlini and Florian Tramer and Eric Wallace and Matthew Jagielski and Ariel Herbert-Voss and Katherine Lee and Adam Roberts and Tom Brown and Dawn Song and Ulfar Erlingsson and Alina Oprea and Colin Raffel},
      year={2021},
      eprint={2012.07805},
      archivePrefix={arXiv},
      primaryClass={cs.CR}
}

@misc{adversarial-training,
      title={Recent Advances in Adversarial Training for Adversarial Robustness}, 
      author={Tao Bai and Jinqi Luo and Jun Zhao and Bihan Wen and Qian Wang},
      year={2021},
      eprint={2102.01356},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@misc{adversarial-input-randomization,
      title={Mitigating Adversarial Effects Through Randomization}, 
      author={Cihang Xie and Jianyu Wang and Zhishuai Zhang and Zhou Ren and Alan Yuille},
      year={2018},
      eprint={1711.01991},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}

@misc{adversarial-regularization,
      title={Improving DNN Robustness to Adversarial Attacks using Jacobian Regularization}, 
      author={Daniel Jakubovitz and Raja Giryes},
      year={2019},
      eprint={1803.08680},
      archivePrefix={arXiv},
      primaryClass={cs.LG}
}

@article{adversarial-detection,
author = {Ahmadi, Morteza and Dianat, Rouhollah and Amirkhani, Hossein},
year = {2021},
month = {03},
pages = {1-30},
title = {An adversarial attack detection method in deep neural networks based on re-attacking approach},
volume = {80},
journal = {Multimedia Tools and Applications},
doi = {10.1007/s11042-020-10261-5}
}

